Methodology for standard cell compliance and detailed placement for triple patterning lithography

As the feature size of semiconductor process further scales to sub-16nm technology node, triple patterning lithography (TPL) has been regarded one of the most promising lithography candidates. M1 and contact layers, which are usually deployed within standard cells, are most critical and complex parts for modern digital designs. Traditional design flow that ignores TPL in early stages may limit the potential to resolve all the TPL conflicts. In this paper, we propose a coherent framework, including standard cell compliance and detailed placement to enable TPL friendly design. Considering TPL constraints during early design stages, such as standard cell compliance, improves the layout decomposability. With the pre-coloring solutions of standard cells, we present a TPL aware detailed placement, where the layout decomposition and placement can be resolved simultaneously. Our experimental results show that, with negligible impact on critical path delay, our framework can resolve the conflicts much more easily, compared with the traditional physical design flow and followed layout decomposition.

==> doc/algo.tex <==

\section{Algorithms}
\label{sec:algo}

In this section we propose our algorithms about the detailed placement scheme.

\subsection{Decomposability Checking}

As shown in Fig. \ref{fig:printability_checker}, the checking of decomposability can be implemented through shortest path searching.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.5\textwidth]{printability_checker}
  \caption{~Decomposability checker with shortest path algorithm.}
  \label{fig:printability_checker}
\end{figure}

\subsection{Detailed Placement Perturbation}

Given an initial cell placement, cells are first sorted in the topological order (i.e., from left to right).
We then start from the first cell and set its orientation to each of two possible choices.
For each partial solution, we process the second cell and set its orientation to each of two choices.
In this way, the algorithm proceeds in a dynamic programming fashion.
Alternate coloring of timing critical paths.

\subsection{Speedup Checking}

Since the checking would be called several times during placement perturbation,
the runtime of checking is critical.
Here we explain several speedup techniques.



==> doc/cover.tex <==

\twocolumn[
\normalsize
\begin{@twocolumnfalse}

Dear ICCAD Technical Program Chair,

\ \\
We are submitting this article as the camera-­‐ready version of ICCAD’13.

In the following, we summarize the differences between this version and the previously submitted version.

\begin{itemize}
  \item
  {
    We include authors, affiliation, and acknowledgment.
  }
  \item
  {
    We use ACM LaTex template, while in previous version we used IEEE LaTex template.
  }
  \item
  {
    Add references: [2][11].
  }
  \item
  {
    Some review comments have been addressed:
    \begin{itemize}
      \item
      {
        We have revised the explanation for Algorithm 1.
      }
      \item
      {
        For Fig. 5, we have made it clear that the six gates are picked up as most commonly used, not all gates in the library.
      }
    \end{itemize}
  }
  \item
  {
    Typos have been corrected:
    \begin{itemize}
      \item
      {
        ``a indecomposable 4-clique conflict structure''
        $\rightarrow$
        ``an indecomposable 4-clique conflict structure''
      }
      \item
      {
        ``has been scaled it to''
        $\rightarrow$
        ``has been scaled to''
      }
      \item
      {
        ``each two cell pair''
        $\rightarrow$
        ``each cell pair''
      }
    \end{itemize}
  }
\end{itemize}

Thank you.

\ \\
Best regards,

\ \\
Bei Yu, Xiaoqing Xu, Jhih-Rong Gao, David Z. Pan

\end{@twocolumnfalse}
]



==> doc/old_dplace.tex <==
\section{Detailed Placement Algorithms}
\label{sec:dplace}

\subsection{Decomposability Checking}
As shown in Fig. \ref{fig:printability_checker}, the checking of decomposability can be implemented through shortest path searching.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.5\textwidth]{printability_checker}
  \caption{~Decomposability checker with shortest path algorithm.}
  \label{fig:printability_checker}
\end{figure}

\subsection{Detailed Placement Perturbation}

Given an initial cell placement, cells are first sorted in the topological order (i.e., from left to right).
We then start from the first cell and set its orientation to each of two possible choices.
For each partial solution, we process the second cell and set its orientation to each of two choices.
In this way, the algorithm proceeds in a dynamic programming fashion.
Alternate coloring of timing critical paths.

\subsection{Cells Speading}

This sub-problem can be formulated as an integer linear programming (ILP).

\subsection{Speedup Checking}

Since the checking would be called several times during placement perturbation,
the runtime of checking is critical.
Here we explain several speedup techniques.


